An Integrated Progressive Hedging and Benders Decomposition with Multiple Master Method to Solve the Brazilian Generation Expansion Problem

This paper exploits the decomposition structure of the large-scale hydrothermal generation expansion planning problem with an integrated modified Benders Decomposition and Progressive Hedging approach. We consider detailed and realistic data from the Brazilian power system to represent hourly chronological constraints based on typical days per month and year. Also, we represent the multistage stochastic nature of the optimal hydrothermal operational policy through co-optimized linear decision rules for individual reservoirs. Therefore, we ensure investment decisions compatible with a nonanticipative (implementable) operational policy. To solve the large-scale optimization problem, we propose an improved Benders Decomposition method with multiple instances of the master problem, each of which strengthened by primal cuts and new Benders cuts generated by each master's trial solution. Additionally, our new approach allows using Progressive Hedging penalization terms for accelerating the convergence of the method. We show that our method is 60\% faster than the benchmark. Finally, the consideration of a nonanticipative operational policy can save 7.64\% of the total cost (16.18\% of the investment costs) and significantly improve spot price profiles.

==> table_bounds.tex <==
\begin{table}[h]
\caption{Comparison of the bounds of each algorithm}
\label{tab:bounds}
%\resizebox{\textwidth}{!}{
\begin{tabular}{ccc}
\hline
\textbf{Algorithm}                & \textbf{Lower Bound} & \textbf{Upper Bound} \\ \hline
TBD & $z^k$                   & $\mathcal{I}^T\hat{x}^k + Q(\hat{x}^k)$                \\
BDMM    & $\max\limits_{s\in\mathcal{S}} \{z^k_s\}$                   & $\min\limits_{s\in\mathcal{S}}\{ \mathcal{I}^T\hat{x}^k_s + Q(\hat{x}^k_s)\}$                \\
r-BDMM                              & $\sum\limits_{s=1}^{S} p_s\zeta^k_s$                   & $\min\limits_{s\in\mathcal{S}}\{ \mathcal{I}^T\hat{x}^k_s + Q(\hat{x}^k_s)\}$                \\ \hline
\end{tabular}%}
\end{table}
